Transfer Learning for Scene Text Recognition in Indian Languages

Scene text recognition in low-resource Indian languages is challenging because of complexities like multiple scripts, fonts, text size, and orientations. In this work, we investigate the power of transfer learning for all the layers of deep scene text recognition networks from English to two common Indian languages. We perform experiments on the conventional CRNN model and STAR-Net to ensure generalisability. To study the effect of change in different scripts, we initially run our experiments on synthetic word images rendered using Unicode fonts. We show that the transfer of English models to simple synthetic datasets of Indian languages is not practical. Instead, we propose to apply transfer learning techniques among Indian languages due to similarity in their n-gram distributions and visual features like the vowels and conjunct characters. We then study the transfer learning among six Indian languages with varying complexities in fonts and word length statistics. We also demonstrate that the learned features of the models transferred from other Indian languages are visually closer (and sometimes even better) to the individual model features than those transferred from English. We finally set new benchmarks for scene-text recognition on Hindi, Telugu, and Malayalam datasets from IIIT-ILST and Bangla dataset from MLT-17 by achieving 6%, 5%, 2%, and 23% gains in Word Recognition Rates (WRRs) compared to previous works. We further improve the MLT-17 Bangla results by plugging in a novel correction BiLSTM into our model. We additionally release a dataset of around 440 scene images containing 500 Gujarati and 2535 Tamil words. WRRs improve over the baselines by 8%, 4%, 5%, and 3% on the MLT-19 Hindi and Bangla datasets and the Gujarati and Tamil datasets.

==> 5Resultsa.tex <==
\begin{table}[t]
\resizebox{0.8\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & CRNN-CRR & CRNN-WRR & STAR-Net-CRR & STAR-Net-WRR \\
\midrule
English & 77.13 & 38.21 & {\bf 86.04} & {\bf 57.28} \\
Gujarati & 94.43 & 81.85 & {\bf 97.80} & {\bf 91.40}\\
Hindi & 89.83 & 73.15 & {\bf 95.78} & {\bf 83.93}\\
Bangla & 91.54 & 70.76 & {\bf 95.52} & {\bf 82.79}\\
Tamil & 82.86 & 48.19 & {\bf 95.40} & {\bf 79.90}\\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{Character Recognition Rate (CRR) and Word
Recognition Rate (WRR) of CRNN and STAR-Net on Synthetic Datasets.}
\label{tab:results_synthetic}
\vspace{-2mm}
\end{table}
\section{Results}\label{sec:results}
In this section, we discuss the results of our experiemnts with i) individual models for each language, ii) the transfer learning models from English to two Indian languages, and iii) the transfer learning models from one Indian language to another.
\begin{table}[ht]
\resizebox{0.8\textwidth}{!}
{%
\centering
\begin{tabular}{crrcrrcrr}
\toprule
Language & Dataset & No. of Images & Model & CRR  & WRR \\%& STAR-Net-CRR & STAR-Net-WRR \\
%& & & (ours,~\cite{mathew2017benchmarking}) & (ours,~\cite{mathew2017benchmarking}) & &\\
\midrule
Gujarati &   ours    & 125 & CRNN (ours) & 84.93 & {\bf 64.80} \\
         &       &     & STAR-Net (ours) & {\bf 85.63} & 64.00 \\
         % 531 = 371 + 160 (0.3) real dataset images
\midrule
 &  &  & Mathew et al.~\cite{mathew2017benchmarking} &  75.60 & 42.90\\%,  & 78.72 & {\bf 46.60} \\{\bf 78.84},
Hindi & IIIT-ILST & 1150 & CRNN (ours) & {\bf 78.84} & 46.56\\
 &  &  & STAR-Net (ours) & 78.72 & {\bf 46.60}\\
\midrule
Hindi & MLT-19 & 3766 & CRNN (ours) & {\bf 86.56} & 64.97\\
 &  &  & STAR-Net (ours) & 86.53 & {\bf 65.79}\\
\midrule
 &  &  & Bušta et al.~\cite{buvsta2018e2e} &   68.60 & 34.20\\%,  & 78.72 & {\bf 46.60} \\{\bf 78.84},
Bangla & MLT-17 & 673 & CRNN (ours) & 71.16 & 52.74 \\
 &  &  & STAR-Net (ours) & {\bf 71.56} & {\bf 55.48} \\ %cleaned images = 656
\midrule
Bangla & MLT-19 & 3691 & CRNN (ours) &  81.93 & 74.26 \\
 &  &  & STAR-Net (ours) & {\bf 82.80} & {\bf 77.48}\\
% Bangla & MLT-19 & 3935 & CRNN (ours) &  {\bf 67.50} & {\bf 35.23} \\
% &  &  & STAR-Net (ours) & 64.08 & 30.68\\
 % cleaned images = 3691
\midrule
Tamil & ours  & 500 & CRNN (ours) & {\bf 84.27} & {\bf 66.06} \\
      &   &      & STAR-Net (ours) &  81.28 & 58.18 \\
      % 2200 =  1540 + 660 real dataset images 
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{CRR and WRR of our models on Real Datasets.}
\label{tab:results_real}
\vspace{-2mm}
\end{table}
\begin{comment}
\begin{table}[ht]
\resizebox{\textwidth}{!}
{%
\centering
\begin{tabular}{crrcrrcrr}
\toprule
Language & Dataset & No. of Images & CRNN-CRR  & CRNN-WRR & STAR-Net-CRR & STAR-Net-WRR \\
& & & (ours,~\cite{mathew2017benchmarking}) & (ours,~\cite{mathew2017benchmarking}) & &\\
\midrule
Hindi & IIIT-ILST & 1150 & {\bf 78.84}, 75.60 & 46.56, 42.90 & 78.72 & {\bf 46.60} \\
      & MLT-2019 & 3766 & {\bf 86.56} & 64.97 & 86.53 & {\bf 65.79} \\
Bangla & MLT-2019 & 3935 & {\bf 64.31} & {\bf 28.51} & 61.34 & 24.82 \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{CRR and WRR of CRNN and STAR-Net on Real Datasets.}
\label{tab:results_real}
\vspace{-4mm}
\end{table}
\end{comment}

{\bf Performance of Individual Models:} In Table~\ref{tab:results_synthetic} and~\ref{tab:results_real}, we present the results of our experiments with individual models for each language. As noted in Table~\ref{tab:results_synthetic}, the CRNN model achieves the Character Recognition Rates (CRRs) and Word Recognition Rates (WRRs) of i) 77.13\% and 38.21\% in English and ii) above $82\%$ and $70\%$ on the synthetic dataset of all the Indian languages (refer to columns 1 and 2 of Table~\ref{tab:results_synthetic}). The low accuracy on the synthetic test set is due to the presence of $>1200$ different fonts (refer Section~\ref{sec:datasets}). Nevertheless, using a large number of fonts in training helps in generalizing the model for real settings~\cite{Jaderberg14c,gupta2016synthetic}. The STAR-Net achieves remarkably better performance than CRNN on all the datasets, with the CRRs and WRRs above $95.40$ and $79.90$ for Indian languages. The reason for this is spatial attention mechanism and powerful residual layers, as discussed in Section~\ref{sec:models}. As shown in column 1 of Table~\ref{tab:results_synthetic}, the WRR of the model trained on Gujarati is highest, followed by Hindi and Bangla and is lowest for Tamil. This is interestingly in the same order as of the language complexity, as discussed in Section~\ref{sec:datasets}. The CRR and WRR of STAR-net also follow this order (columns 3 and 4 of Table~\ref{tab:results_synthetic})\footnote{The CRR of the CRNN model is sightly lower than that of Bangla, perhaps due to fewer fonts and shorter average word-length in Bangla than Hindi (refer Table~\ref{tab:synth_data}).}. %The probable reason for this is availability of lesser number of fonts in Bangla as compared to Hindi (refer Table~\ref{tab:synth_data}). %As we discuss next, the trend is as per average word-length and language complexity for the real datasets.

Table~\ref{tab:results_real} depicts the performance of our models on the real datasets. At first, we observe that the STAR-Net achieves slightly better WRR than CRNN, whereas the latter reaches a slightly better CRR. Next, please note that Mathew et al.~\cite{mathew2017benchmarking} meet the CRR and WRR of $75.60\%$ and $42.90\%$ on the IIIT-ILST Hindi dataset, over which we observe an increase of $3.24\%$ and $3.7\%$ with our models. This happens because we remove the non-Unicode and zero-width Unicode characters from the text while rendering our training datasets. We share two new baselines for the MLT-19 Hindi dataset\footnote{The word-level recognition task is not part of the competition, and individual language results for end-to-end text spotting are not shared by Nayef et al.~\cite{nayef2019icdar2019}.}. For the two Hindi datasets, STAR-Net produces slightly better WRR than CRNN, whereas the latter is better at the character level. For the MLT-17 Bangla dataset, STAR-Net achieves $2.95\%$ improvement on CRR and a stunning $21.28\%$ gain in WRR over the results reported by Bušta et al.~\cite{buvsta2017deep}. For MLT-19 Bangla dataset, we set two baselines similar to Hindi. For the two Bangla datasets, STAR-Net performs better than CRNN in terms of both CRR and WRR. For Tamil dataset, we observe that CRNN performs much better than STAR-Met for both CRR and WRR. Overall, we achieve better scores than previous works. Also, note that STAR-Net performs better than CRNN for $7$ recognition rates ($4$ WRR, $3$ CRR), and the latter performs better for $5$ recognition rates ($2$ WRR, $3$ CRR). As we discuss in the next sub-section, transfer learning help us further improve these results.%We also observe that STAR-Net achieves slightly better WRRs than the CRNN model for the Hindi and Tamil datasets. However, we note that the CRRs of STAR-Net are lower than CRNN models on all of the datasets except Tamil. This happens perhaps due to the over-fitting of STAR-Net to synthetic datasets. \sanjana{Finetuning on real datasets may handle this issue.} OR As we discuss in the next sub-section, transfer learning help tackle these issues.


\begin{comment}
\begin{table}[ht]
\resizebox{\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & CRNN-CRR (individual target) & CRNN-WRR (individual target) \\
\midrule
Gujarati  $\longrightarrow$  Hindi & 0.92 (0.89) & 0.73 (0.73)\\
Hindi $\longrightarrow$ Bangla &  &  \\
Bangla $\longrightarrow$ Tamil &  &  \\
Tamil $\longrightarrow$ Bangla &  &  \\
Bangla $\longrightarrow$ Hindi &  &  \\
Hindi $\longrightarrow$ Gujarati & 0.95 (0.94) & 0.84 (0.81) \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{CRR and WRR of CRNN on Synthetic Datasets upon Transfer Learning.}
\label{tab:results_transferLearning}
\end{table}
\end{comment}

\begin{table}[ht]
\resizebox{0.8\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & CRNN-CRR & CRNN-WRR & STAR-Net-CRR & STAR-Net-WRR \\
& (individual target) & (individual target) & (individual target) & (individual target)\\
\midrule
English $\longrightarrow$ Gujarati & 92.71 ({\bf 94.43}) & 77.06 ({\bf 81.85}) & 97.50 ({\bf  97.80}) & 90.90 ({\bf 91.40}) \\
English $\longrightarrow$ Hindi &  88.11 ({\bf 89.83}) & 70.12 ({\bf 73.15}) & 94.50 ({\bf 95.78}) & 80.90 ({\bf 83.93}) \\%correct these later if any mistake
\midrule
Gujarati  $\longrightarrow$  Hindi & {\bf 91.98} (89.83) & 73.12 ({\bf 73.15}) & {\bf 96.12} (95.78) &  {\bf 84.32} (83.93)\\
Hindi $\longrightarrow$ Bangla & 91.13 ({\bf 91.54}) & 70.22 ({\bf 70.76}) & {\bf 95.66} (95.52) & {\bf 82.81} (82.79) \\
Bangla $\longrightarrow$ Tamil & 81.18 ({\bf 82.86}) & 44.74 ({\bf 48.19}) & {\bf 95.95} (95.40) & {\bf 81.73} (79.90) \\
\midrule
Tamil $\longrightarrow$ Bangla & 90.37 ({\bf 91.54}) & 67.61 ({\bf 70.76}) & {\bf 95.63} (95.52) & 82.74 ({\bf 82.79}) \\
Bangla $\longrightarrow$ Hindi & {\bf 91.16} (89.83) & 72.06 ({\bf 73.12}) & {\bf 96.06} (95.78) &  {\bf 84.06} (83.93) \\
Hindi $\longrightarrow$ Gujarati & {\bf 95.36} (94.43) & {\bf 84.21} (81.85) & {\bf 98.08} (97.80) & {\bf 92.81} (91.40) \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{CRR and WRR of our models on Synthetic Datasets upon Transfer Learning.}
\label{tab:results_transferLearning_STAR-Net_synth}
\vspace{-2mm}
\end{table}
{\bf Performance with Transfer Learning:} We first experiment with synthetic datasets to improve the models in Table~\ref{tab:results_synthetic} from the previous sub-section. We mention the best individual model results from the last sub-section in brackets for comparison. We begin with the English models as the base because the models have trained on over $1200$ fonts and $17M$ word images as discussed in Section~\ref{sec:datasets}, and are hence generic. However, in the first two rows of the table, we note that transferring the layers from the model trained on the English dataset to Gujarati and Hindi is inefficient. This happens because Indic scripts have many different visual as well as slightly different n-gram characteristics from English, as discussed in Section~\ref{sec:datasets}. We then note that as we try to apply transfer learning among Indian languages with CRNN (rows 3-8, columns 1-2 in the table), only some combinations work well. We, however, note that with STAR-Net (rows 3-8, columns 3-4 in the table), transfer learning helps improving results on the synthetic dataset from a simple language to complex language (rows 3-5), as well as from a tricky language to a simple one (rows 6-8). However, we note that transfer learning from a simple language to a complex is more effective. Thus, we fine-tune the best STAR-net models (rows 3-5 and 8 in the table) obtained in this stage on the real datasets with the methodology described in the previous section.
\begin{table}[ht]
\resizebox{0.7\textwidth}{!}
{%
\centering
\begin{tabular}{crrcrrcrr}
\toprule
Language & Dataset & No. of Images & Model & CRR & WRR \\
 & & & & (individual best) & (individual best) \\%& STAR-Net-CRR & STAR-Net-WRR \\
%& & & (ours,~\cite{mathew2017benchmarking}) & (ours,~\cite{mathew2017benchmarking}) & &\\
\midrule
English$\longrightarrow$Gujarati &  ours & 125 & STAR-Net & 68.48 ({\bf 85.63}) & 60.18 ({\bf 64.80})\\% CHANGED58.48 29.37
English$\longrightarrow$Hindi & IIIT-ILST & 1150 & STAR-Net & 77.43 ({\bf 78.84}) & 44.81 ({\bf 46.60})\\ %based on 5M exp, please update these later for 2.5M exp
\midrule
Hindi $\longrightarrow$ Gujarati &  ours  & 125 & STAR-Net & {\bf 88.47} (85.63) & {\bf 69.60} (64.80) \\
%         &       &     & CRNN & 40.98 & 12.94 \\
\midrule
% &  &  & Mathew et al.~\cite{mathew2017benchmarking} &  75.60 & 42.90\\%,  & 78.72 & {\bf 46.60} \\{\bf 78.84},
Gujarati$\longrightarrow$Hindi & IIIT-ILST & 1150 & STAR-Net & {\bf 79.12} (78.84) & {\bf 47.79} (46.60)\\
% &  &  & STAR-Net & 78.72 & {\bf 46.60}\\
Gujarati$\longrightarrow$Hindi & MLT-19 & 3766 & STAR-Net & {\bf 89.42} (86.56) & {\bf 72.96} (65.79)\\%\\64.97\\
% &  &  & STAR-Net & 86.53 & {\bf 65.79}\\
\midrule
% &  &  & Bušta et al.~\cite{buvsta2018e2e} &   68.60 & 34.20\\%,  & 78.72 & {\bf 46.60} \\{\bf 78.84},
Hindi $\longrightarrow$ Bangla & MLT-17 & 673 & STAR-Net & {\bf 72.16} (71.56)  & {\bf 57.01} (55.48)\\
% &  &  & STAR-Net &  & \\
Hindi $\longrightarrow$ Bangla & MLT-19 & 3691 & STAR-Net &  {\bf 82.91} (82.80) & {\bf 78.02} (77.48) \\
% &  &  & STAR-Net & 61.34 & 24.82\\
%      & MLT-2019 & 3766 & {\bf 86.56} & 64.97 & 86.53 & {\bf 65.79} \\
%Bangla & MLT-2019 & 3935 & {\bf 64.31} & {\bf 28.51} & 61.34 & 24.82 \\
\midrule
Bangla $\longrightarrow$Tamil & ours  & 500  & STAR-Net & 80.97 ({\bf 84.27}) & 57.87 ({\bf 66.06}) \\%& CRNN (ours) & 57.91 & 20.82 \\
%      &   &      & STAR-Net (ours) & {\bf 59.45} & {\bf 24.89} \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{CRR and WRR of our models on Real Datasets upon Transfer Learning.}
\label{tab:results_tl_real}
\vspace{-2mm}
\end{table}
\vspace{-2mm}
\begin{comment}
\begin{table}[ht]
\resizebox{0.7\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & STAR-Net-CRR (individual target) & STAR-Net-WRR (individual target) \\
\midrule
Gujarati  $\longrightarrow$  Hindi &  () &  ()\\
Hindi $\longrightarrow$ Bangla & () & () \\
%Bangla $\longrightarrow$ Tamil & 95.95 (95.40) & 81.73 (79.90) \\
Tamil $\longrightarrow$ Bangla & () & () \\
Bangla $\longrightarrow$ Hindi &  () &  () \\
%Hindi $\longrightarrow$ Gujarati & 98.08 (97.80) & 92.81 (91.40) \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{CRR and WRR of of STAR-Net on Real Datasets upon Transfer Learning.}
\label{tab:results_transferLearning_STAR-Net_real}
\end{table}
\end{comment}
In the first two rows of Table~\ref{tab:results_tl_real}\footnote{the best individual model results on real datasets from the previous sub-section (Table~\ref{tab:results_real} are copied in brackets for comparison.}, we again notice that fine-tuning the models with layers transferred from English does not help improve results in Indian languages. However, we see that the STAR-Net layers transferred from one Indic dataset to another set new recognition benchmarks for our Gujarati dataset, IIIT-ILST and MLT-19 Hindi datasets, MLT-17 and MLT-19 Bangla datasets. We, however, note in the last row of the table that the transfer learning is ineffective from Bangla to Tamil. The reason for this may be the extremity in the hardness of the Tamil language as discussed in Section~\ref{sec:datasets}. With the increase in the public datasets of one of the Indian languages and better transfer learning techniques, or with the rise in real Tamil datasets for fine-tuning, we hope to achieve improved results for Tamil as the future work of our research.

\begin{figure}[ht]%[!t]
    \centering
    \includegraphics[trim=0 335 0 0,width=0.8\linewidth]{images/HinViz.jpg}%
    \vspace{0.1mm}
    \includegraphics[trim=0 340 0 0,width=0.8\linewidth]{images/GujViz.jpg}%
    \caption{Visualization of initial layers of CNN in the i) top: CRNN models trained on Hindi and transferred from English$\longrightarrow$ Hindi, and Gujarati$\longrightarrow$ Hindi, and ii) bottom: STAR-Net models trained on Gujarati, English$\longrightarrow$Gujarati and Hindi$\longrightarrow$ Gujarati. Red boxes indicate the regions where the transferred model with English as the base is mostly activated with white, whereas the other two are not.}
    \label{fig:visualizations}
    \vspace{-2mm}
\end{figure}
{\bf Features Visualization:} In Figure~\ref{fig:visualizations} for the CRNN model, we visualize the learned CNN layers of the individual Hindi model, the "English$\longrightarrow$Hindi" model, and the "Gujarati$\longrightarrow$Hindi" model. The red boxes are the areas where the first four CNN layers of the model transferred from English to Hindi are different from the other two models. This again strengthens our claim that transfer from the English reading model to any Indian language dataset is inefficient. We also notice a similar trend for the Gujarati STAR-Net models, though the initial CNN layers look very close to word images. This also demonstrates the better learnability of STAR-net compared to CRNN, as observed in the previous sub-sections.

==> 5Resultsprev.tex <==
\section{Results}\label{sec:results}

\begin{table}[ht]
\resizebox{0.7\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & CRNN-CRR & CRNN-WRR & STARNET-CRR & STARNET-WRR \\
\midrule
Gujarati & 0.94 & 0.81 & 97.80 & 91.40\\
Hindi & 0.89 & 0.73 & 95.70 & 81.90\\
Bangla & 0.91 & 0.70 & 95.52 & 82.79\\
Tamil & 0.82 & 0.48 & 95.40 & 79.90\\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{Character Recognition Rate (CRR) and Word
Recognition Rate (WRR) of CRNN on synthetic data.}
\label{tab:results}
\end{table}

\begin{table}[ht]
\resizebox{0.7\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & CRNN-CRR (individual target) & CRNN-WRR (individual target) \\
\midrule
Gujarati  $\longrightarrow$  Hindi & 0.92 (0.89) & 0.73 (0.73)\\
Hindi $\longrightarrow$ Bangla &  &  \\
Bangla $\longrightarrow$ Tamil &  &  \\
Tamil $\longrightarrow$ Bangla &  &  \\
Bangla $\longrightarrow$ Hindi &  &  \\
Hindi $\longrightarrow$ Gujarati & 0.95 (0.94) & 0.84 (0.81) \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{Character Recognition Rate (CRR) and Word
Recognition Rate (WRR) of CRNN on synthetic data upon Transfer Learning.}
\label{tab:results_transferLearning}
\end{table}

\begin{table}[ht]
\resizebox{0.7\textwidth}{!}
{%
\centering
\begin{tabular}{crrrr}
\toprule
Language & STARNET-CRR (individual target) & STARNET-WRR (individual target) \\
\midrule
Gujarati  $\longrightarrow$  Hindi &  (95.70) &  (81.90)\\
Hindi $\longrightarrow$ Bangla & 95.66 (95.52) & 82.81 (82.79) \\
Bangla $\longrightarrow$ Tamil & 95.95 (95.40) & 81.73 (79.90) \\
Tamil $\longrightarrow$ Bangla & 95.63 (82.79) & 82.74 (82.79) \\
Bangla $\longrightarrow$ Hindi &  (95.70) &  (81.90) \\
Hindi $\longrightarrow$ Gujarati & 98.08 (97.80) & 92.81 (91.40) \\
English $\longrightarrow$ Gujarati & 97.50 (97.80) & 90.90 (91.40) \\
%\hline
%{\bf Total}  & $\mathbf{1515}$ & $\mathbf{23848}$ & $\mathbf{140,106}$ \\
\bottomrule
\end{tabular}
}
\caption{Character Recognition Rate (CRR) and Word
Recognition Rate (WRR) of CRNN on synthetic data upon Transfer Learning.}
\label{tab:results_transferLearning_starnet}
\end{table}
